Nonparametric Factor Analysis and Beyond

Nearly all identifiability results in unsupervised representation learning inspired by, e.g., independent component analysis, factor analysis, and causal representation learning, rely on assumptions of additive independent noise or noiseless regimes. In contrast, we study the more general case where noise can take arbitrary forms, depend on latent variables, and be non-invertibly entangled within a nonlinear function. We propose a general framework for identifying latent variables in the nonparametric noisy settings. We first show that, under suitable conditions, the generative model is identifiable up to certain submanifold indeterminacies even in the presence of non-negligible noise. Furthermore, under the structural or distributional variability conditions, we prove that latent variables of the general nonlinear models are identifiable up to trivial indeterminacies. Based on the proposed theoretical framework, we have also developed corresponding estimation methods and validated them in various synthetic and real-world settings. Interestingly, our estimate of the true GDP growth from alternative measurements suggests more insightful information on the economies than official reports. We expect our framework to provide new insight into how both researchers and practitioners deal with latent variables in real-world scenarios.

==> sections/theory_old.tex <==
\section{From identification in distribution to identification in observation}
\label{sec:identification}
We assume that a researcher observe the distribution of $\{X_1, X_2,\ldots,X_k\}$ from a random sample. Putting the estimation of the population distribution $P_{X_1, X_2,\ldots,X_k}$ from the random sample aside, we face a key identification challenge: How to determine the distribution $P_{X_1, X_2,\ldots,X_k,Z}$ from the observed distribution $P_{X_1, X_2,\ldots,X_k}$. Here we use a general nonparametric identification result in the measurement error literature.

\begin{restatable}{assumption}{assump0}
\label{assumption 3.0} 
There exists a random variable $Z$ with support $\mathcal{X}^{ \ast }$ such that  
\begin{eqnarray}  \nonumber
&&P_{X_1, X_2,\ldots,X_k,Z} \\ \nonumber
&=& P_{X_1|Z} f_{X_2|Z} \times ... \times P_{X_k|Z} P_{Z}.
\end{eqnarray}\normalsize
\normalsize 
\end{restatable}

We may consider the observables $(X_1, X_2,\ldots,X_k)$ as measurements of $Z$. Here we use \citep{hu2008instrumental} to show the uniqueness of $f(X_1, X_2,\ldots,X_k,Z)$. We assume three of the $k$ measurements are informative enough for the results in \citep{hu2008instrumental}. We assume
\begin{restatable}{assumption}{assump1}
\label{assumption 3.1} The joint distribution of $(X_1, X_2,\ldots,X_k,Z)$ with $k \geq 3$ admits a bounded density with respect to the product measure of
some dominating measure defined on their supports. All marginal and conditional densities are also bounded.
\end{restatable}
Before introducing more assumptions, we define an integral operator corresponding to $f_{X_1\vert X^{ \ast }}$, which maps $f_{X^{ \ast }}$ over support $\mathcal{X}^{ \ast }$ to $f_{X_1}$ over support $\mathcal{X}^{ 1 }$. Suppose that we know both $f_{X^{ \ast }}$ and $f_{X_1}$ are bounded and integrable. We define $\mathcal{L}_{b n d}^{1} \left (\mathcal{X}^{ \ast }\right )$ as the set of bounded and integrable functions defined on $\mathcal{X}^{ \ast }$, i.e.,
\begin{eqnarray}\nonumber
&&\mathcal{L}_{b n d}^{1} \left (\mathcal{X}^{ \ast }\right ) \\ \nonumber
&=&\left \{g :\int _{\mathcal{X}^{ \ast }}\left \vert g (x^{ \ast })\right \vert   dx^{ \ast } <\infty \;, \;\sup_{x^{ \ast } \in \mathcal{X}^{ \ast }}\left \vert g (x^{ \ast })\right \vert  <\infty \right \}. \label{equ 060}
\end{eqnarray}\normalsize
\normalsize
The linear operator can be defined as
\begin{eqnarray}L_{X_1\vert X^{ \ast }} &  : & \mathcal{L}_{b n d}^{1} \left (\mathcal{X}^{ \ast }\right ) \rightarrow \mathcal{L}_{b n d}^{1} \left (\mathcal{X}^1\right ) \label{equ 070} \\
\left (L_{X_1\vert X^{ \ast }} h\right ) \left (x\right ) &  = & \int _{\mathcal{X}^{ \ast }}f_{X_1\vert X^{ \ast }} (x\vert x^{ \ast })h (x^{ \ast })  dx^{ \ast } . \nonumber \end{eqnarray}\normalsize  
\normalsize
In order to identify the unknown distributions, we need the observables to be informative so that the following assumptions hold.
\begin{restatable}{assumption}{assump2}
\label{assumption 3.2}The operators $L_{X_1\vert X^{ \ast }}$ and $L_{X_2\vert X_1}$ are injective.\protect\footnote{ $L_{X_2\vert X_1}$ is defined in the same way as $L_{X_1\vert X^{ \ast }}$ in equation (\ref{equ 070}).}
\end{restatable}

\begin{restatable}{assumption}{assump3}
\label{assumption 3.3}For all $\overline{x}^{ \ast } \neq \widetilde{x}^{ \ast }$ in $\mathcal{X}^{ \ast }$, the set $\left \{x^3 :f_{X_3\vert X^{ \ast }} \left (x^3\vert \overline{x}^{ \ast }\right ) \neq f_{X_3\vert X^{ \ast }} \left (x^3\vert \widetilde{x}^{ \ast }\right )\right \}$ has positive probability.
\end{restatable}

\begin{restatable}{assumption}{assump4}
\label{assumption 3.4}There exists a known functional $M$ such that $M\left [f_{X_1\vert X^{ \ast }} \left ( \cdot \vert x^{ \ast }\right )\right ] =x^{ \ast }$ for all $x^{ \ast } \in \mathcal{X}^{ \ast }$.
\end{restatable}
\noindent The functional $M$ may be the mean, mode, medium, or another quantile of the distribution $f_{X_1\vert X^{ \ast }} \left ( \cdot \vert x^{ \ast }\right ) $. The identification result may be summarized as follows:

\begin{restatable}{theorem}{HuSc2008} \label{HuSc2008}
\citep{hu2008instrumental} Under assumptions \ref{assumption 3.0}, \ref{assumption 3.1}, \ref{assumption 3.2}, \ref{assumption 3.3}, and \ref{assumption 3.4} in the Appendix, the joint distribution $f_{X_1, X_2,\ldots,X_k}$ uniquely determines the joint distribution $f_{X_1, X_2,\ldots,X_k,Z}$, which satisfies 
\begin{equation}\label{equ 200}
f_{X_1, X_2,\ldots,X_k,Z} = f_{X_1|Z} f_{X_2|Z} \cdot ... \cdot f_{X_k|Z} f_{Z}. 
\end{equation}
\end{restatable}

This identification result only needs three measurements. Therefore, the conditional independence may be relaxed to 
\begin{equation*} 
f_{X_1, X_2,\ldots,X_k,Z} = f_{X_1|Z} f_{X_2|Z} f_{X_3,\ldots,X_k,Z}. 
\end{equation*}

In the remaining discussion, we still use the conditional independence in equation (\ref{equ 200}) because we are interested in the common element $Z$ across all the observables. This identification result implies that if we have qualified measurements $X_1$, $X_2$ and $X_3$, we are able to provide a consistent estimator of $f_{X_1, X_2,\ldots,X_k,Z}$ from a sample of $(X_1, X_2,\ldots,X_k)$. 

\subsection{Uncorrelated deviations and identification in observation} 
Next, we argue that draws of $Z$ are locally identified in the sense that there is no observationally equivalent uncorrelated deviation from these draws. 

Let  $Z_i$ be a random draw of $Z$ in observation $i$ and we define \textit{an uncorrelated deviation} from that draw as 
\begin{equation} \label{indep deviation}
Z_i+\delta_i \quad \mbox{with} \quad \mathbb{E}(Z_i  \delta_i)=\mathbb{E}( \delta_i)=0
\end{equation}

where $(Z_i,\delta_i)$ is a i.i.d. random draw from the joint distribution of $(Z,\delta)$. 
Notice that if we replace $Z_i$ with $Z_i+\delta_i$ as the new common element, the variance of the common element becomes $var(Z) + var(\delta)$. 
% \begin{equation}
% var(Z) + var(\delta)
% \end{equation}
That means the variance of the uncorrelated deviation must be different from that of the original $Z$, i.e., $var(Z)$. The distribution of $Z+\delta$ must be different from that of $Z$. These two different distributions cannot lead to the same observed distribution,  $f_{X_1, X_2,\ldots,X_k}$, because Theorem \ref{HuSc2008} implies that  $f_{X_1, X_2,\ldots,X_k}$ uniquely determines $f_{Z}$, including its variance $var(Z)$. In other words, $Z+\delta$ and $Z$ cannot be observationally equivalent given the sample of $(X_1, X_2,\ldots,X_k)$. Therefore, the draws of $Z$ are locally identified in the following sense:

\begin{restatable}{theorem}{ThmID} \label{Theorem id local}
Suppose that the assumptions in Theorem \ref{HuSc2008} hold. Given an observed sample $\{X^1_i, X^2_i,\ldots,X^k_i \}$, which is a subset of the infeasible full sample $\{X^1_i, X^2_i,\ldots,X^k_i, Z_i \}$, no uncorrelated deviation from latent draws $Z_i$, defined in equation (\ref{indep deviation}), is observationally equivalent to $Z_i$.  
\end{restatable}

Notice that we only use the identified variance of the latent $Z$ to make this argument. The results in Theorem \ref{HuSc2008} implies that all the moments of the latent $Z$ are identified. Therefore, such a local identification result as in Theorem \ref{Theorem id local} should hold for more general deviations than the uncorrelated deviations defined in equation (\ref{indep deviation}).

Furthermore, we may look at this problem from a different angle. Suppose we insert generated draws $\hat{X}^*_i$ in the sample $\{X^1_i, X^2_i,\ldots,X^k_i \}$ to obtain $\{X^1_i, X^2_i,\ldots,X^k_i, \hat{X}^*_i \}$. And we also suppose that the conditional independence in equation (\ref{equ 200}) holds with the generated draws, i.e.,
\begin{equation*} \nonumber
f_{X_1, X_2,\ldots,X_k,\hat{X}^*} = f_{X_1|\hat{X}^*} f_{X_2|\hat{X}^*} \times ... \times f_{X_k|\hat{X}^*z} f_{\hat{X}^*}. 
\end{equation*}
In this case, even if $\hat{X}^*_i$ is not equal to the true $Z_i$ in the infeasible full sample $\{X^1_i, X^2_i,\ldots,X^k_i, Z_i \}$, our inserted $\hat{X}^*_i$ will be observationally equivalent to the true $Z_i$ because Theorem \ref{HuSc2008} guarantees that the distributions  $f_{X_1|Z}$,  $f_{X_2|Z}$, and $ f_{X_3,\ldots,X_k,Z}$ are uniquely determined by the observed $f_{X_1, X_2,\ldots,X_k}$. Even if $\hat{X}^*_i \neq Z_i$, we can still correctly estimate $f_{X_1|Z}$,  $f_{X_2|Z}$, and $ f_{X_3,\ldots,X_k,Z}$ using sample $(X_i^1, X_i^2,\ldots,X_i^k,\hat{X}^*_i)_{i=1,2,\ldots,N}$ with inserted $\hat{X}^*_i$, instead of the true values $Z_i$. 

Moreover, Theorem \ref{Theorem id local} implies that if we add a noise $\delta_i$ to the inserted $\hat{X}^*_i$, where $\delta_i$ is an uncorrelated deviation from $\hat{X}^*_i$, the conditional independence fails when $\hat{X}^*_i$ is replaced with $\hat{X}^*_i+\delta_i$. That means the inserted draws $\hat{X}^*_i$ are locally unique among uncorrelated deviations. 

The identification result in Theorem \ref{Theorem id local} can be extended to the case where $\delta_i$ is uncorrelated with $Z_i$ conditional on the observables $(X_1, X_2,\ldots,X_k)$ because the conditional distribution $f_{Z|X_1, X_2,\ldots,X_k}$ is identified by Theorem \ref{HuSc2008}. We define \textit{a conditionally uncorrelated deviation} from $Z_i$ as $Z_i+\delta_i$ with 
\begin{align} \label{cond indep deviation}
    &\mathbb{E}(Z_i \delta_i \, \vert \, X_i^1, X_i^2,\ldots,X_i^k) \\
    = &\mathbb{E}( \delta_i \, \vert \, X_i^1, X_i^2,\ldots,X_i^k) =0,
\end{align}
where $(Z_i ,\delta_i , X_i^1, X_i^2,\ldots,X_i^k)$ is a i.i.d. random draw from their corresponding joint distribution. The variance, and therefore distribution, of $Z_i+\delta_i $ conditional on $(X_1, X_2,\ldots,X_k)$ is different from those of $f_{Z|X_1, X_2,\ldots,X_k}$. Theorem \ref{HuSc2008} implies that they must correspond to different $f_{X_1, X_2,\ldots,X_k}$. Therefore, there is no observationally equivalent conditionally uncorrelated deviation from latent draws $Z_i$. We summarize this extension as follows:
\begin{restatable}{theorem}{ThmID2} \label{Theorem id2}
Suppose that the assumptions in Theorem \ref{HuSc2008} hold. Given an observed sample $\{X^1_i, X^2_i,\ldots,X^k_i \}$, which is a subset of the infeasible full sample $\{X^1_i, X^2_i,\ldots,X^k_i, Z_i \}$, no \textit{conditionally uncorrelated deviation} from latent draws $Z_i$, defined in equation (\ref{cond indep deviation}), is observationally equivalent to $Z_i$. 
\end{restatable}


%Suppose our identification results suggest that our estimates $\hat{X}^*_i $ should have the same distribution (and variance) as $Z_i$. Then the sample moments of $\hat{X}^*_i $ should converge to the true moments. We may make a convergence argument as follows:

%\begin{restatable}{theorem}{Cons}  %\label{consistency}
%Suppose that the estimator $\hat{X}^*_i  = Z_i + \delta_i $ for $i=1,2,\ldots,N$ satisfies 
%\begin{eqnarray} %\label{condition -- deviation}
% \frac{1}{N} \sum_{i=1}^{N} Z_i \delta_i = o_p(1).
%\end{eqnarray}
%Then, the consistency of the sample variance of $\hat{X}^*_i$  implies that for any $\epsilon>0$, the sample proportion of large deviations goes to zero, i.e.,
%\begin{equation*}
%P_N \left ( \left | \hat{X}^*_i - Z_i \right |>\epsilon \right ) := \frac{1}{N} \sum_{i=1}^{N} I( |\delta_i| > \epsilon)= o_p(1).
%\end{equation*}
%\end{restatable}
%\noindent We leave the details in the Appendix.

\subsection{Point identification in observation}
The identification with respect to uncorrelated deviations is still not enough to pin down the value of the unobserved in each observation. Here we provide a point identification argument for the value of the unobserved variable in each observation. Let $X^{(i)}= ( X_1^{(i)}, X_2^{(i)},\ldots,X_k^{(i)})^T $ and $Z^{(i)}$ be observed and unobserved variables describing subject $i$, respectively. Define the population of random variables $\{X_i, Z_i\}$ as set
$$
\mathcal{P}_{X,Z} = \{{(x, z)}^{(i)} :   i= 1,2,\ldots, \infty \} .
$$

Suppose that one never observes two subjects alike. Then the mapping from observed $X$ to unobserved $Z$ is a function, i.e., a set of ordered pairs $(x,z)$ in which no two different ordered pairs have the same first coordinate. Therefore, such a function can uniquely determine unobserved $z$ from observed $x$ for each subject. Formally, we assume
\begin{restatable}{assumption}{AssumpLeaf}
\label{assumption leaf} 
No two different subjects in the population are observationally identical, i.e., for any $ {(x, z)}^{(i)}$ and ${(x, z)}^{(j)}$ in $\mathcal{P}_{X,Z}$, 
 $i \neq j$ implies  $x^{(i)} \neq x^{(j)}$.
\end{restatable}
Under this property, the mapping defined by set $\mathcal{P}_{X,Z} $, i.e., the population of $\{X_i, Z_i\}$, is a function mapping from $X$ to $Z$. Notice that $x^*_i$ is not necessarily distinct for different subject $i$.  

Define such a function as 
$$
Z = G(X).
$$
Then the identification of distribution $f(X,Z)$ implies the identification of function $G$. In fact, we have 
$$
G(X) = \mathbb{E}[Z| X].
$$
The property in Assumption \ref{assumption leaf} implies that the distribution of $Z$ degenerates conditional on $X$. Therefore, any location, such as conditional mean or median, of the distribution $f(Z|X)$ can reveal the value of $x^*_i$ in each observation $i$. Therefore, we can extend the identification in distribution in in Theorem \ref{HuSc2008} as follows:

\begin{restatable}{theorem}{Thmid} \label{Theorem id}
Suppose that the assumptions in Theorem \ref{HuSc2008} and Assumption \ref{assumption leaf} hold. Given an observed sample $\{X^1_i, X^2_i,\ldots,X^k_i \}$, which is a subset of the infeasible full sample $\{X^1_i, X^2_i,\ldots,X^k_i, Z_i \}$, the realization of $Z_i$ in observation $i$ is uniquely determined by the realization of $\{X^1_i, X^2_i,\ldots,X^k_i \}$ in the observation. In particular,
$$
x^*_i = \mathbb{E}[Z| X^1_i=x^1_i, X^2_i=x^2_i,\ldots,X^k_i=x^k_i ].
$$
\end{restatable}

In most applications, Assumption \ref{assumption leaf} is satisfied because we usually do not have two observations which are exactly the same. In the case where this happens, the point identification result here implies that researchers need to obtain more measurement or observables so that identification of unobservable is possible. Here we provide an example to illustrate the identification. 

Suppose we have for $j=1,2,3$ and $X_4$:
\begin{eqnarray}
X_j &=& f^j(Z) + \epsilon_j, \nonumber \\
X_4 &=& \Phi(Z/3) * (-1)^ {I(\epsilon_4>0.5)}, \nonumber
\end{eqnarray}
where $\Phi$ is the cumulative distribution function of the standard normal distribution and $(X_1,X_2,X_3)$ satisfies the assumptions in Theorem \ref{HuSc2008}. In particular, we assume $(\epsilon_1,\epsilon_2,\epsilon_3,\epsilon_4,Z)$ are jointly independent. So distribution $f(X_1,X_2,X_3)$ uniquely determines distribution $f(X_1,X_2,X_3, Z)$. Assumption \ref{assumption leaf} is satisfied because 
$$
Z = 3 * \Phi ^{-1} (|X_4|)
$$
The value of $(\epsilon_1,\epsilon_2,\epsilon_3)$  can be determined by a given value of $(X_1,X_2,X_3,Z)$. When $\epsilon_4$ is a 0-1 binary random variable,  the value of $\epsilon_4$ can also be determined by a given value of $(X_2,X_3,X_4,Z)$.

Notice that 
\begin{align*}
    &p(X_1,X_2,X_3,X_4) \\
    = &\int p(X_1| Z) p(Z,X_2,X_3,X_4)dZ.
\end{align*}
Given that $p(X_1| Z)$ is identified from $p(X_1,X_2,X_3)$ and its corresponding integral operator is injective, distribution $p(Z,X_2,X_3,X_4)$ is also identified. Therefore, the whole distribution $p(X_1,X_2,X_3,X_4,Z)$. In fact, one can show that 
$$
\mathbb{E}[Z|X_1,X_2,X_3,X_4] = 3 * \Phi ^{-1} (|X_4|).
$$
Therefore, the realization of $Z$ is uniquely determined and also estimable in each observation.


We also have the following results to ensure that the dimension of the recovered unobserved variable cannot be further reduced under continuity.

\begin{restatable}{theorem}{Reduce1D}\label{thm:reduc1d}
    A one-to-one function $f: \mathbb{R}^n \rightarrow \mathbb{R}$ cannot be continuous. Therefore, the dimentionality of $\mathbb{R}^n$ can't be reduced to that of $\mathbb{R}$ under the continuity. 
\end{restatable}



\begin{restatable}{theorem}{ReduceKD}\label{thm:reduckd}
    A one-to-one function $f: \mathbb{R}^n \rightarrow \mathbb{R}^k$ with $k<n$ can't be continuous. Therefore, the dimentionality of $\mathbb{R}^n$ can't be reduced to that of $\mathbb{R}^k$ under the continuity.  
\end{restatable}

These results have important implications for our identification strategy. They imply that the unobserved variable $Z$ must retain its intrinsic dimensionality when being recovered from observed data under continuity assumptions. In other words, we cannot hope to represent a higher-dimensional unobserved variable using a lower-dimensional observed counterpart without losing continuity or injectivity. This reinforces the necessity of our approach in maintaining the dimensionality of $Z$ during estimation to ensure accurate and unique recovery of its realizations, which is especially essential for cases with multivariate latent variables.
